Privacy-Preserving Filtering for Event Streams

Many large-scale information systems such as intelligent transportation systems, smart grids or smart buildings collect data about the activities of their users to optimize their operations. To encourage participation and adoption of these systems, it is becoming increasingly important that the design process take privacy issues into consideration. In a typical scenario, signals originate from many sensors capturing events involving the users, and several statistics of interest need to be continuously published in real-time. This paper considers the problem of providing differential privacy guarantees for such multi-input multi-output systems processing event streams. We show how to construct and optimize various extensions of the zero-forcing equalization mechanism, which we previously proposed for single-input single-output systems. Some of these extensions can take a model of the input signals into account. We illustrate our privacy-preserving filter design methodology through the problem of privately monitoring and forecasting occupancy in a building equipped with multiple motion detection sensors.

==> texFiles/7_examples.tex <==
%!TEX root =  ../dpEventFiltering.tex

\subsection{Example: Events Generated by Markovian Dynamics}		%\label{eq: example}

%For example, individual users could be generating an event when entering or leaving one of $N$ locations, 
%or when starting or stopping one of $N$ activities. In the context of non-intrusive load monitoring in a single
%household\todo{ref?}, users could in fact be appliances responsible for sharp power consumption changes,
%and we would like to hide the usage of some of these appliances.

We illustrate through a simple example that performance improvement over the ZFE mechanism is 
possible when we take into account additional public information about the input signals, as described in the 
previous subsections.
%
Consider a server (central computer, clerk in an administrative office, etc.) processing jobs submitted by customers, 
and which can be either $\mathtt{idle}$ or $\mathtt{busy}$. An event is recorded when
the server switches from one state to another. One way of representing this system is via the Markov 
chain model with $4$ states shown on Fig. \ref{fig: Markov chain example}, with an event being generated when 
the server enters the intermediary states $\mathtt{s_1}$ and $\mathtt{s_2}$, in which it can only stay for one time period.
%As a concrete example, consider the following model. We have two locations and denote by $x_{i,t}$
%the number of people at location $i = 1,2$ at time $t$. The overall state of the system at time $t$ is 
%thus $x_t = (x_{1,t}, x_{2,t})$. Two sensors generate the following signals: $u_{i,t}=+1$ when
%a person enters location $i=1,2$ from outside, and $u_{i,t}=-1$ when a person leaves location $i$ to
%go outside. A person can also move directly between the two locations, but there is no sensor to detect 
%these transitions. Suppose that the state evolution is described by a Markov chain in the stationary
%regime, with known transition probabilities as given on Fig. ??. \todo{Still to do}
The events recorded at the transition times should be kept private. For example, in a cloud computing environment,
processing times and patterns could provide some information about the jobs submitted by a customer
that he or she does not want to disclose \cite{Kadloor:TSP12:privateScheduling}. On the other hand, we assume
that the parameters $\alpha, \beta$ governing the transition probabilities and shown on Fig. \ref{fig: Markov chain example}
are public information.

\begin{figure}
\centering
\includegraphics[height=4cm]{graphics/simpleMarkovChain}
\caption{Transition probabilities for the Markov chain example.
The numbering of states $1$ to $4$ is the one used to express the z-spectrum \eqref{eq: spectrum Markov chain}.
We assume $\alpha, \beta \notin \{0,1\}$, in which case the chain is ergodic.
The stationary probabilities are then $p_1 = \beta/q$, $p_2 = p_4 = \alpha \beta / q$, $p_3 = \alpha / q$, 
with $q = \alpha + \beta + 2 \alpha \beta$.} 
\label{fig: Markov chain example}
\end{figure}

For a general discrete Markov chain $\{x_t\}_t$ with $N$ states, we can assume without loss of generality that the state space
is the set of $N$-dimensional unit vectors denoted $\{e_1, \ldots, e_N\}$, with $e_{ij} = \delta_{ij}$. Denote the 
$N$-by-$N$ transition probability matrix $\Pi$, with elements $\Pi_{ij} = \mathbb P(x_{t+1} = e_i | x_t = e_j)$. 
Assume moreover that the chain is \textcolor{red}{ergodic} and stationary, and introduce the column vector $p$, 
where $p_i = \mathbb P(x_t = e_i)$, with $\Pi p = p$. Note that with this encoding of the states we have 
$\mathbb E[x_t] = \mathbf p$. For convenience we also introduce the $0$-mean sequence
$\tilde x_t = x_t - \mathbf{p}$, taking values in $\{\tilde e_1,\ldots,\tilde e_N\}$ with $\tilde e_i = e_i - \mathbf p$.
Finally, let $D = \text{diag}(p_1,\ldots,p_N)$. Then one can show that \cite{Bilardi:Comm83:MCspectrum} 
\begin{equation}	\label{eq: spectrum Markov chain}
P_x(z) = pp^T + H(z) C H(z^{-1})^T = p p^T + P_{\tilde x}(z),
\end{equation}
where $H(z) = (zI-\Pi)^{-1}$ and $C = D - \Pi D \Pi^T$. 
%
Using this formalism to represent the server dynamics above via a stationary Markov chain, with $N = 4$, the
two stationary signals generated by the server entering the intermediate states  $\mathtt{s_1}$ and $\mathtt{s_2}$ 
encoded here as $e_2$ and $e_4$ are $u_{1,t} = e_2^T x_t, u_{2,t} = e_4^T x_t,$, so that
$P_u(z) = \begin{bmatrix} e_2^T \\ e_4^T \end{bmatrix} P_x(z) \begin{bmatrix} e_2 & e_4 \end{bmatrix}$.
%Note that with the transition probabilities given on \textcolor{red}{Fig. ??} the stationary state probabilities
%are $D = \text{diag}...$

Suppose now that we want to release a filtered version of the two-dimensional input signal $u$, with  the 
specified filter $F$ given by the following $2 \times 2$ transfer matrix for example
\[
F = \ldots
\]



 %%%%%%%%%%%%
 
%Starting from the sequence of visited state $x_t$, one could be interested in certain events generated when
%a state is entered or left, for example
%\[
%u_{1,t} = e_j^T(x_t - x_{t-1})
%\]
%is equal to $1$ at the period $t$ when $x_t$ enters state $e_j$, $-1$ when it leaves $e_j$, and $0$ otherwise.
%Its PSD is simply $P_{u_1}(z) = e_j^T (1-z^{-1})^2 P_{\tilde x}(z) e_j$. Hence, let $u$ be a vector valued
%signal of interest obtained from such filtering operations on $x$, and let $P_u(z)$ be its power spectral density.
%As before we assume that $\mathbb E[u_t] = 0$ by subtracting and processing independently the known mean 
%if necessary.

%
%
%
%Let $X_k$ be a discrete stationary Markov chain with $N$ states. Without loss of generality, we let the state space be
%the set of $N$-dimensional unit vectors denoted $\{e_1,\ldots,e_N\}$.
%%For $N$ the number of states of a Markov chain, let $e_1,\ldots, e_N$ denote the $N$-dimensional unit vectors.
%%We encode the state $X_k$ by letting take its values in $\{e_1,\ldots,e_N\}$. 
%Then we have the state-space representation
%\begin{align}		\label{eq: state-space MC}
%X_{k+1} = \Pi X_k + V_{k+1},
%\end{align}
%where $\Pi_{ij} = P(X_{k+1} = e_j | X_k = e_i)$ and $V_{k}$ is a martingale difference sequence (white noise) with respect 
%to the filtration $\mathcal F_k = \sigma \{X_0,\ldots,X_k\}$. That is, $V_k$ is $\mathcal F_k$-measurable and 
%$\mathbb E[V_{k+1} | \mathcal F_k] = 0$. Recall that as a consequence we have $\mathbb E[V_k V^T_l] = 0$ for $k \neq l$.
%Moreover, it is straightforward to compute that
%\[
%\begin{cases} 
%R_x[l] = \mathbb E[X_k X_{k-l}^T] = \Pi^l D, & l \geq 0 \\
%R_x[l] = D (\Pi^T)^l, & l < 0.
%\end{cases}
%\]
%We deduce
%\begin{align*}
%C = \mathbb E[V_k V_k^T] &= \mathbb E[(X_{k+1} - \Pi X_k) (X_{k+1} - \Pi X_k)^T] \\
%&= D + \Pi D \Pi^T - \Pi \mathbb E[ X_k X_{k+1}^T] - \mathbb E[ X_{k+1} X_{k}^T \Pi^T] \\
%&= D - \Pi D \Pi^T.
%\end{align*}
%In view of \eqref{eq: state-space MC} we obtain the PSD of $x$ as
%\[
%P_x(z) = H(z) C H(z^{-1})^T,
%\]
%where $H(z) = (zI-\Pi)^{-1}$.
%
%We can record events triggered by certain transitions. For example, events associated to entering
%or leaving state $j$ can be recorded as
%\[
%u_t = e_j^T (X_t - X_{t-1}),
%\]
%which gives $+1$ if the state becomes $j$ at $t$, $-1$ if the state leaves $j$ at $t-1$, and $0$ otherwise,
%including if the state remains in $j$.

%%%%%%%%%%%%%%%%%%%
% CDC paper

%
%
%\vspace{1cm}
%
%
%%We conclude with a brief example. 
%Consider approximating the filter
%$
%%F(z) = \frac{1}{s(z)+p}
%F(z) = \frac{1+0.995 z^{-1}}{1-0.995 z^{-1}},
%$
%%with $s(z)$ the bilinear transformation $s(z) = 2 \frac{1-z^{-1}}{1+z^{-1}}$, and $p$ a parameter. 
%with the privacy parameters set to $\epsilon = \ln 3$, $\delta = 0.05$.
%The (wide-sense stationary) input signal is assumed to be binary valued, i.e., $u_t \in \left\{ \pm \frac{1}{2} \right\}$ for all $t$, with zero mean and power spectral
%density 
%$
%%P_u(z) = \frac{3/4}{(z-1/2)(z^{-1}-1/2)}.
%P_u(z) = \frac{3/4}{\left(1-\frac{1}{2}z^{-1}\right)\left(1-\frac{z}{2}\right)}.
%$
%Such a signal can be generated by a two-state Markov chain in the stationary regime, with transition probability matrix
%\[
%\begin{bmatrix}
%3/4 & 1/4 \\ 1/4 & 3/4
%\end{bmatrix},
%\]
%one state corresponding to the input $-1/2$, and the other state corresponding to the input $1/2$, see, e.g., \cite{Brighenti09_MCspectrum}.
%In this context we can imagine that the transitions are generated by individual users, and we want to prevent an adversary analyzing the trace 
%$\{(Fu)_t\}_t$ to infer with confidence in which state the chain was at a particular time.
%
%We designed four mechanism: LZF, LMMSE with $G$ optimized based on (\ref{eq: optimization LMMSE-M}), 
%DF with $G$ optimized based on (\ref{eq: optimization DF-M}), and DF with the same $G$ as for the LMMSE mechanism.
%The DF estimators introduce a $5$-period delay in the production of the estimate (finite impulse response equalizers were implemented here,
%based on \cite{Voois96_delayDFE}).
%Typical sample paths for these four mechanisms are shown on Fig. \ref{fig: sample paths}.
%The theoretical root MSE (RMSE) for the LZF and (non-causal) LMMSE mechanisms are $8.82$ and $7.43$ respectively.
%We see that the DF mechanisms significantly reduces the fluctuations in the produced output. 
%Moreover, the LMMSE pre-filter $G$ leads to a clearly better performance for the DF mechanism than the one  
%based on (\ref{eq: optimization DF-M}) in this case. 
%The magnitude of the frequency response $|G(e^{j \omega})|$ is shown on Fig. \ref{fig: Bode plots} for both filters. 
%%One can observe from the magnitude of the frequency response $|G(e^{j \omega})|$ of both filters 
%We observe
%that the cutoff of the LMMSE pre-filter occurs much earlier, taking into
%account the fact that $F$ filters the high frequencies of $u$ anyway, and this helps reduce the degradation
%due to the privacy-preserving noise $n$.
%
%\begin{figure}
%\centering
%%\includegraphics[width=\linewidth]{graphics/samplePaths2}
%\includegraphics[height=10cm]{graphics/samplePaths2}
%\caption{Sample Paths for four mechanisms. From top to bottom: LZF, LMMSE, DF with $G$ optimized based on (\ref{eq: optimization DF-M}), 
%and DF with the same $G$ as for the LMMSE mechanism. The original non-private output is shown as the thick blue line.} %dotted blue line.}
%\label{fig: sample paths}
%\end{figure}
%%
%\begin{figure}
%\includegraphics[width=\linewidth]{graphics/bodePlots}
%\caption{Magnitude of the frequency reponse $|G(e^{j \omega})|$ for $G$ designed based on (\ref{eq: optimization LMMSE-M}) (top), 
%and based on (\ref{eq: optimization DF-M}) (bottom).}
%\label{fig: Bode plots}
%\end{figure}







